Dynamical Programming for off-the-grid dynamic Inverse Problems

In this work we consider algorithms for reconstructing time-varying data into a finite sum of discrete trajectories, alternatively, an off-the-grid sparse-spikes decomposition which is continuous in time. Recent work showed that this decomposition was possible by minimising a convex variational model which combined a quadratic data fidelity with dynamical Optimal Transport. We generalise this framework and propose new numerical methods which leverage efficient classical algorithms for computing shortest paths on directed acyclic graphs. Our theoretical analysis confirms that these methods converge to globally optimal reconstructions which represent a finite number of discrete trajectories. Numerically, we show new examples for unbalanced Optimal Transport penalties, and for balanced examples we are 100 times faster in comparison to the previously known method.

==> conditional_expectation.tex <==
%! TEX root = ../main.tex

\layout{\pagebreak}
\section{Conditional expectation lemma}\label{app: conditional expectation proof}
\begin{lmm}[{Lemma~\ref{lmma: independent conditional expectation}}]
	Suppose $X$ is an $\Filtration$-measurable random variable and $Z\perp X, \Filtration$ (\ie\ $Z$ is independent of $X$ and $\Filtration$) is another random variable. Then, for all integrable Borel measurable functions $g$
	\begin{equation}
		\E(g(X,Z)|\Filtration) = G(X) \qtext{where} G(x) \eqdef \E(g(x,Z)).
	\end{equation}
\end{lmm}
\begin{proof}
	Let $Y$ be an arbitrary $\Filtration$-measurable random variable. We are required to show that $\E\left[YG(X)\right] = \E\left[Yg(X,Z)\right]$.
	Recall that if $X,Y\perp Z$, then the joint law $\P(X=x,Y=y,Z=z)$ factorises into $\P(X=x,Y=y)\P(Z=z)$. We can therefore compute
	\begin{align}
		\E\left[Yg(X,Z)\right] &= \int yg(x,z)\xdif\P(X=x,Y=y,Z=z)
		\\&= \iint yg(x,z)\xdif\P(X=x,Y=y)\xdif\P(Z=z) & (X,Y\perp Z)
		\\&= \int y\left[\int g(x,z)\xdif\P(Z=z)\right] \xdif\P(X=x,Y=y) & (\text{Fubini's theorem})
		\\&= \E\left[Y G(X)\right]
	\end{align}
	as required.
\end{proof}


==> fwcv.tex <==
%! TEX root = ../main.tex
\section{Frank-Wolfe convergence}\label{sec: FW convergence}
While Theorem~\Rref{thm: structure of E} guarantees an analytical structure of minimisers, we must now choose a reconstruction algorithm which is capable of taking advantage of this structure. As previously stated, we will use a variant of the Frank-Wolfe algorithm to take advantage of the sparse structure of reconstructions. \edit{}{Most of this section will be presented in the general Frank-Wolfe framework with additional discussion clarifying its application in the specific setting of Section~\Rref{sec: generalisation}.} In particular, we minimise a convex function $\op{E}\colon D\to\xR$ with a well-defined choice of \emph{linear minimisation oracle} $\LO\colon D\to D$ satisfying
\begin{equation}\label{eq: general linear oracle}
	\forall \tilde\cm\in D,\qquad
	\LO(\tilde\cm) \in \argmin_{\cm\in D} \IP{\op{E}'(\tilde\cm)}{\cm}
\end{equation}
where $\op{E}'$ is the Gateaux derivative of $\op{E}$ on $D$. With this notation, the variant of Frank-Wolfe that we will use is given in Algorithm~\Rref{alg: inexact FW}. In particular, we use the ``sliding'' variant which has been shown to have a much greater performance in practical applications \cite{denoyelleSlidingFrankWolfeAlgorithm2019}.


In the context of Section~\Rref{sec: generalisation}, one can verify that $\op{E}'(\cm) = \op{F}'(\cm) + w$ where $\op{F}'\colon D\to \Cb(\HG)$ is defined by
\begin{equation}
	\forall\cm\in D,\qquad \op{F}'(\cm)= \left[(\h,\g)\mapsto\sum_{j=0}^T \h(t_j)\eta_j(\g(t_j))\right]\qtext{where} \eta_j \eqdef A_j^*\nabla \op{F}_j(A_j\cmt{t_j}).
\end{equation}
It can be verified that $\op{F}'$ is a representation of the Gateaux derivative of $\op{F}$. The following lemma confirms that the linear oracle is both well-defined and can be expressed by a potentially simpler optimisation problem over the space $\HG$.
\begin{lmm}\label{lmma: well defined linear oracle}
	Suppose $\varphi,w\colon\HG\to\ci{0}{+\infty}$ are lower semi-continuous. If $\inf_{\hg\in\HG}\varphi(\hg)>0$ and either $\varphi$ or $w$ have compact sub-levelsets, then there exists a choice of $\LO(\tilde\cm)$ such that
	\begin{equation}\label{eq: exact linear oracle}
		\LO(\tilde\cm) \in\{0\} \cup \enscond{\varphi(\hg^*)^{-1}\delta_{\hg^*}}{ \hg^* \in \argmin_{\hg\in\HG} \frac{\eta(\hg) + w(\hg)}{\varphi(\hg)}}.
	\end{equation}
	where $\eta(\h,\g) \eqdef \sum_{j=0}^T \h(t_j)\eta_j(\g(t_j))\in \Cb(\HG)$.
\end{lmm}
\begin{proof}
	Recall the definition of $\LO$, 
	\begin{equation}
		\LO(\tilde\cm) \in \argmin_{\cm\in D} \tilde{\op{E}}(\cm) \qtext{where} \tilde{\op{E}}(\cm) \eqdef \int_{\HG}\left(\eta +w\right)\xdif\cm.
	\end{equation}
	The properties of $D$ come from Lemma~\Rref{lmma: extreme point computation}, in particular $D$ is convex, closed and bounded, so $\inf_{\cm\in D}\int_\HG\eta\xdif\cm>-\infty$ and $\tilde{\op{E}}$ is lower semi-continuous (Lemma~\Rref{thm: Fatou's lemma}). It is therefore well-posed to consider minimisers of $\tilde{\op{E}}$. We show that there is a choice $\LO(\tilde\cm)=\cm^*\in\Ext D$.
	
	\begin{description}
		\item[Case $D$ is compact] If $\varphi$ has compact sub-levelsets, then $D$ is compact by Lemma~\Rref{lmma: extreme point computation}. Bauer's principle therefore states that there exists a point
		\begin{equation}
			\cm^*\in\Ext{D} \qtext{such that} \tilde{\op{E}}(\cm^*) = \inf_{\cm\in D}\tilde{\op{E}}(\cm).
		\end{equation}
		
		\item[Else] Otherwise, $w$ has compact sub-levelsets, so the sub-levelset 
		\begin{equation}
			U \eqdef \enscond{\cm\in D\quad}{\quad \tilde{\op{E}}(\cm) \leq 1}
		\end{equation}
		is compact by Theorem~\Rref{thm: compact sub-levelsets}, convex, and non-empty because $0\in D$, $\tilde{\op{E}}(0)=0$. Application of Bauer's principle now gives a point $\cm^*\in\Ext{U}$, to complete the proof we will confirm $\cm^*\in\Ext{D}$. 
		
		Suppose for contradiction that there exists $\cm_0,\cm_1\in D\setminus\{\cm^*\}$ with $\cm^*\in\oi{\cm_0}{\cm_1}$. Without loss of generality, we assume that $\cm^*=\frac{1}{2}\cm_0+\frac{1}{2}\cm_1$ and we define
		\begin{equation}
			\forall \lambda\in\ci01,\qquad \cm_\lambda\eqdef\lambda\cm_1 + (1-\lambda)\cm_0\in D,\qquad \cm_{\frac12} = \cm^*.
		\end{equation}
		Consider the function $f(\lambda) = \tilde{\op{E}}(\cm_\lambda)$, which is linear and $f(\frac12)=\tilde{\op{E}}(\cm^*) \leq \tilde{\op{E}}(0)=0$. As $f$ is continuous, there exists $\epsilon>0$ with $f(\frac12\pm\epsilon)\leq \frac12$. We conclude that $\cm_{\frac12\pm\epsilon}\in U$ and $\cm^*\in\oi{\cm_{\frac12-\epsilon}}{\cm_{\frac12+\epsilon}}$, contradicting the assumption that $\cm^*\in\Ext{U}$.
	\end{description}
	In both cases we see there is a choice $\LO(\tilde\cm)=\cm^*\in\Ext D$. Finally, by Lemma~\Rref{lmma: extreme point computation} we have 
	\begin{equation}
		\Ext D = \{0\}\cup\enscond{\varphi(\hg)^{-1}\delta_{\hg}}{\varphi(\hg)<+\infty},
	\end{equation} 
	so \eqref{eq: exact linear oracle} is just the required statement
	\begin{equation}
		\cm^* \in\argmin_{\cm\in \Ext{D}}\tilde{\op{E}}(\cm) \subset \{0\}\cup\enscond{\varphi(\hg^*)^{-1}\delta_{\hg^*}}{\hg^*\in \argmin_{\hg\in\HG} \tilde{\op{E}}\left(\varphi(\hg)^{-1}\delta_\hg\right)}.
	\end{equation}
\end{proof}

\begin{algorithm}
	\begin{algorithmic}[1]
		\State Choose $ \cm^0\in D$ with $\op{E}(\cm^0)<+\infty$, $n\gets0$, 
		\Repeat
		\State $\ep^{n+1} \gets \LO(\cm^n)$ \Comment{linear oracle} \label{alg: inexact step}
		\State $\lambda_n\gets \argmin_{\lambda\in\ci01} \op{E}((1-\lambda)\cm^n + \lambda \ep^{n+1})$ \Comment{exact linesearch}
		\State Choose $\cm^{n+1}$ such that $\op{E}(\cm^{n+1}) \leq \op{E}((1-\lambda_n)\cm^n + \lambda_n \ep^{n+1})$ \Comment{Sliding step}
		\State $n\gets n+1$
		\Until{converged}
	\end{algorithmic}
	\caption{Sliding Frank-Wolfe algorithm}\label{alg: inexact FW}
\end{algorithm}

\subsection{Choice of constraint}\label{sec:FW discussion}
A major advantage of Frank-Wolfe / Generalised Conditional Gradient methods is their ability to minimise energies like~\eqref{eq: def of E} while constructing iterates which share the same sparse structure~\eqref{eq: sparse structure} as the minimisers (see for instance \cite{brediesInverseProblemsSpaces2013,boydAlternatingDescentConditional2017,denoyelleSlidingFrankWolfeAlgorithm2019} in the case of point sources recovery).
The method proposed in~\cite{BrediesNumerics} follows that approach, and the core of the algorithm is the minimisation of a linear functional on the level sets of $\creg$ (see~\cite[Prop. 3.6]{BrediesNumerics}). The description of the extreme points of those level sets in~\cite{BrediesBalanced} makes it possible to reformulate that problem as a variational problem on curves.

In the present section, we point out that, while the algorithm derived in \cite{BrediesNumerics} is quite natural, there are many possible ways to define a Frank-Wolfe--based algorithm minimising~\eqref{eq: def of E}.
The example considered there uses the Benamou-Brenier penalty which, recall from Remark~\Rref{rmk: BB energy on curves}, leads to the optimisation problem
\begin{align}
	\min_{\cm \in \MC^+(\HG)} 
	\frac12\sum_{j=0}^T\norm{A_j\cmt{t_j}-\data_j}_2^2 
	+\int_\HG w\xdif\cm\label{bbexample-eq-objfw}\\
	\mbox{where}\quad \forall \g \in \HG, \quad w(\g)\eqdef \alpha + \frac{\beta}{2}\int_0^1|\g'(t)|^2\xdif t. \label{eq:BBalg:w}
\end{align}

The standard Frank-Wolfe procedure consists in iteratively minimising the linearisation of \eqref{bbexample-eq-objfw} on a compact set (for some suitable topology) to yield descent directions. 
At iteration $n$, let $\eta_j\eqdef A_j^*\left(A_j\cmt[\cm^n]{t_j}-\data_j\right)$ denote the linearisation of each summand of the fidelity term. We are led to minimise
\begin{equation}\label{eq: BB linear oracle}
	\min_{\cm \in D}\int_{\HG} \left[\sum_{j=0}^T\eta_j(\g(t_j)) + w(\g)\right]\xdif\cm,
\end{equation}
where $D \subset \MC^+(\HG)$ is a suitably chosen compact convex set which contains the minimisers of $\op{E}$ on $\MC^+(\HG)$. A first choice is to consider the set
\begin{equation}
	D_1\eqdef \enscond{\cm \in \MC^+(\HG)}{\int_{\HG} w\xdif\cm\leq \op{E}(0)},
\end{equation}
which does contain the minimisers of \eqref{bbexample-eq-objfw} since they must satisfy $\int_\HG w\xdif \cm\leq \op{E}(\cm)\leq \op{E}(0)$.
By Lemma~\Rref{lmma: extreme point computation}, the set of extreme points of $D_1$ is 
$\{0\}\cup \enscond{ \frac{\op{E}(0)}{w(\g)}\delta_{\g}}{\g \in \HG}$, which yields the descent direction 
\begin{equation}\label{eq: BB Bredies LO}
	\g^{n+1} \in \argmin_{\g\in\HG} \frac{\sum_{j=0}^T\eta_j(\g_j) + w(\g)}{w(\g)} = \argmin_{\g\in\HG} \frac{\sum_{j=0}^T\eta_j(\g_j)}{w(\g)}.
\end{equation}
That is precisely the descent direction used in~\cite[(4.30)]{BrediesNumerics}, although in that context \eqref{eq: BB linear oracle} is written as a minimisation over $\dm\in\MC^+(\X)$.

On the other hand, alternative choices for $D$ are possible. We propose to use
\begin{equation}
	D_2\eqdef \enscond{\cm \in \MC^+(\HG)}{\int_{\HG} \alpha \xdif\cm\leq \op{E}(0)},
\end{equation}
which contains the minimisers of \eqref{bbexample-eq-objfw} too, since they must satisfy ${\int_\HG \alpha\xdif \cm \leq \int_\HG w\xdif \cm\leq \op{E}(\cm)\leq \op{E}(0)}$.
Applying Lemma~\Rref{lmma: extreme point computation}, we see that the set of extreme points of $D_2$ is 
$\{0\}\cup \enscond{\frac{\op{E}(0)}{\alpha}\delta_{\g}}{\g \in \HG}$, which yields the linear minimisation step
\begin{equation}\label{eq: BB our LO}
	\g^{n+1} \in \argmin_{\g\in\HG} \frac{\sum_{j=0}^T\eta_j(\g_j) + w(\g)}{1} = \argmin_{\g\in\HG} \sum_{j=0}^T\eta_j(\g_j) + w(\g).
\end{equation}
We found \eqref{eq: BB our LO} more convenient than \eqref{eq: BB Bredies LO} as it is amenable to dynamic programming techniques (see Section~\Rref{sec: dynamical programming}). The whole minimisation algorithm is summarised in Algorithm~\Rref{alg: FW}.

\begin{rmrk}
	In measure spaces, compactness is equivalent to boundedness and tightness (Prokhorov's theorem). In both cases, boundedness comes from $\alpha>0$, and tightness comes from the fact that $w$ has compact sub-levelsets. The set $D_1$ is compact by Lemma~\Rref{thm: compact W sublevel}. On the other hand, $D_2$ is only bounded, but sub-levelsets of \eqref{eq: BB linear oracle} are still compact, as argued in Lemma~\Rref{lmma: well defined linear oracle}.
\end{rmrk}

\begin{algorithm}
	\begin{algorithmic}[1]
		\State Choose $ \cm^0=0$, $n\gets0$
		\Repeat
		\State $\eta_j \gets A_j^*(A_j\cmt[\cm^n]{t_j}-\data_j) \in \Co(\bar\Omega)$ \Comment{Gradient of data term}
		\State Compute $\g^{n+1}$ according to \eqref{eq: BB Bredies LO} or \eqref{eq: BB our LO}\Comment{Linear oracle step} \label{alg: BB linear oracle line}
		\State Choose $\ep^{n+1} \propto \delta_{\g^{n+1}} $ such that $\ep^{n+1}\in\Ext{D} $ \Comment{Choice of scaling}
		\State $\cm^{n+1} \gets (1-\lambda_n)\cm^n + \lambda_n \ep^{n+1}$ \Comment{Some stepsize $\lambda_n\in\ci01$}
		\State $n\gets n+1$
		\Until{converged}
	\end{algorithmic}
	\caption{Frank-Wolfe algorithm for the Benamou-Brenier example}\label{alg: FW}
\end{algorithm}


\subsection{Inexact linear oracle}\label{sec: deterministic FW}
While the formula in \eqref{eq: exact linear oracle} requires minimising over a much smaller space than the original formula in \eqref{eq: general linear oracle}, it is still intractable in practical applications. To simplify this further, we consider using an inexact linear oracle estimate in line~\Rref{alg: inexact step} of Algorithm~\Rref{alg: inexact FW}, which we will write as $\ep^{n+1} = \bar{\LO}(\cm^n)\approx \LO(\cm^n)$. In the context of this work, we choose $\bar{\LO}$ to be an exact minimisation over a much smaller discretised space-time domain. \edit{}{The result of \cite[Thm. 1]{Jaggi2013} shows that inexact oracles still leads to convergence whenever the approximation error decreases at a controlled rate. In practice this would correspond to choosing a sufficiently fine discretisation at iteration $n$, relative to the smoothness of $\op{E}$, to guarantee an approximation error of $O(n^{-1})$. Unfortunately the computational complexity of such an approach scales very poorly when trying to approximate $\HG$. For example, a uniform mesh with order $n^{-1}$ resolution leads to a search-space of size $n^{\d(T+1)}$, much too large for a naive search if the number of time frames $T$ is large. To account for this, we relax the requirements of $\bar{\LO}$ in exchange for strengthening the choice of stepsize $\lambda$. A linesearch guarantees both that small steps are made when $\ep^{n+1}$ is a poor choice and large steps are made if $\ep^{n+1}$ is accurate. Asymptotic convergence follows under mild assumptions on the accuracy of $\bar{\LO}$.}

\begin{thrm}\label{thm: inexact FW}
	Suppose $\{\cm^n,\ep^n,\lambda_n\}_{n\in\xN}$ are generated by Algorithm~\Rref{alg: inexact FW} with an inexact oracle $\bar{\LO}$ and there exists $\cm^*\in\argmin_{\cm\in D}\op{E}(\cm)$.
	If $\op{E}$ has bounded curvature, \ie
	\begin{equation}
		C_E\eqdef \sup_{\substack{\cm,\tilde\cm\in D\\\lambda\in\oi01}} \frac{\op{E}((1-\lambda)\cm+\lambda\tilde\cm) - \op{E}(\cm)-\lambda\int_\HG \op{E}'(\cm) \xdif [\tilde\cm-\cm]}{\lambda^2} <+\infty,
	\end{equation}
	and 
	\begin{equation}\label{eq: def of gap}
		\liminf_{n\to+\infty} \gap_n \leq 0\qtext{where} \gap_n\eqdef \IP{\op{E}'(\cm^n)}{\ep^{n+1}-\cm^*},
	\end{equation}
	then $\lim_{n\to+\infty} \op{E}(\cm^n) = \op{E}(\cm^*)$.
\end{thrm}
\begin{proof}
	\todo{We can't just use Jaggi's proof because our error is not relative, he assumes\\ $\gap_n\leq \IP{\op{E}'(\cm^n)}{\LO(\cm^n)-\cm^*}+\delta\lambda$, ours is much more relaxed. Anyway, this is about as short as I can make the proof.}
	Choose $C\in\oi{0}{+\infty}$ to be 
	\begin{equation}\label{eq: def of C}
		C \eqdef \max\left(\tfrac12(\op{E}(\cm^0)-\op{E}(\cm^*)),\ C_E\right).
	\end{equation}
	The convexity of $\op{E}$ implies $\op{E}(\cm^n)+\int_\HG \op{E}'(\cm^n)\xdif[\cm^*-\cm^n] \leq \op{E}(\cm^*)$ for each $n\in\xN$, so for each $\lambda\in\ci01$
	\begin{align}
		\op{E}((1-\lambda)\cm^n+\lambda\ep^{n+1}) &\leq \op{E}(\cm^n) + \lambda\int_\HG \op{E}'(\cm^n)\xdif[\ep^{n+1}-\cm^n] + \frac{C\lambda^2}{2}
		\\&\leq (1-\lambda)\op{E}(\cm^n) + \lambda\left[\op{E}(\cm^*) + \int_\HG \op{E}'(\cm^n)\xdif[\ep^{n+1}-\cm^*]\right] + \frac{C\lambda^2}{2}.
	\end{align}
	Passing to the infimum on the left-hand side and substituting the gap \eqref{eq: def of gap}, we deduce the bound
	\begin{equation}\label{eq: FW linesearch}
		\forall\lambda\in\ci01,\qquad \op{E}(\cm^{n+1})-\op{E}(\cm^*) \leq (1-\lambda)(\op{E}(\cm^n)-\op{E}(\cm^*)) + \lambda \gap_n + \frac{C}{2}\lambda^2.
	\end{equation}
	Recall that, since $\liminf_{n \to \infty}\gap_{n}\leq 0$, there exist a subsequence $(n_k)_{k \in \xN}$ such that $\gap_{n_k}\leq \frac{C}{k}$ for all $k\geq 1$. In \eqref{eq: FW linesearch} we then choose $\lambda=\frac2k$ for $n=n_k$ and $\lambda=0$ else. 
	
	Finally we proceed by induction. Note that $\op{E}(\cm^{n_2})-\op{E}(\cm^*)\leq \op{E}(\cm^{0})-\op{E}(\cm^*)\leq 2C$ by \eqref{eq: def of C}. Next, if for some $k\geq 2$, $\op{E}(\cm^{n_k})-\op{E}(\cm^*)\leq \frac{4C}{k}$, we choose $\lambda = \frac{2}{k}\in\ci01$, then \eqref{eq: FW linesearch} becomes
	\begin{equation}
		\op{E}(\cm^{n_{k+1}}) - \op{E}(\cm^*) \leq \left(1-\frac2k\right)\frac{4C}{k} + \frac2k\frac{C}{k}+\frac{C}{2}\frac{4}{k^2}
		= \frac{4C}{k}\left(1-\frac2k+\frac1k\right)
		\leq \frac{4C}{k}\left(1-\frac1{k+1}\right)
		= \frac{4C}{k+1}.
	\end{equation}
	We conclude by induction that the inequality holds for all $k\geq 2$. By monotonicity, $\lim_{n\to+\infty}\op{E}(\cm^n) = \lim_{k\to+\infty} \op{E}(\cm^{n_k}) = \op{E}(\cm^*)$ as required.
\end{proof}


\subsection{Stochastic inexact linear oracle}\label{sec: random FW}
The main convergence requirement of Theorem~\Rref{thm: inexact FW} is to guarantee $\liminf_{n\to+\infty} \gap_n \leq 0$. Our solution to this is to use random discretisations of $\HG$ so that the inexact variant of Algorithm~\Rref{alg: inexact FW} still converges asymptotically (almost surely), but the complexity of each individual iteration remains low. \edit{}{A similar idea in the setting of stochastic Frank-Wolfe was pursued in \cite{Silveti2020} where their proof relies on what is called Assumption P.8, in our notation this requires the sum $\sum_{n=0}^\infty\lambda_n\gap_n<+\infty$ to be finite almost surely where $\lambda_n$ is chosen deterministically. To apply this algorithm in our setting we would therefore need to bound the magnitude of $\gap_n$ relative to the \apriori\ choice of $\lambda_n$, although it is hard to estimate $\gap_n$ when the minimiser $\cm^*$ is unknown. This is where the linesearch for $\lambda$ again stabilises the convergence of Algorithm~\Rref{alg: inexact FW} despite poor control over $\gap_n$.} This is made formal by the following theorem.

\begin{thrm}\label{thm: inexact stochastic FW}
	Let $\cm^*$ and $\{\cm^n,\ep^n,\lambda_n\}_{n\in\xN}$ be as in Theorem~\Rref{thm: inexact FW} where $\ep^n$ is chosen stochastically. Let $\Filtration^N$ be the filtration generated by $\{\cm^n,\ep^n\}_{0\leq n\leq N}$, and let $\delta\colon\hc{0}{+\infty}\to\ci01$ such that
	\begin{equation}\label{eq: delta condition}
		\forall n\in\xN,\ \epsilon\geq0,\qquad \P(\gap_n \leq \epsilon | \Filtration^n)\geq \delta(\epsilon)\quad \Filtration^n\text{-almost surely}.
	\end{equation}
	If $\op{F}$ has bounded curvature and $\delta(\epsilon)>0$ for all $\epsilon>0$, then $\lim_{n\to+\infty} \op{E}(\cm^n) = \op{E}(\cm^*)$ almost-surely.
\end{thrm}
\begin{proof}
	The first step is to convert the assumption on $\P(\gap_n\leq \epsilon|\Filtration^n)$ into a statement about $\liminf_{n\to+\infty}\gap_n$. For fixed $\epsilon>0$ observe, by sub-additivity and monotone convergence for measures, that
	\begin{multline}
		\P\left[\liminf_{n\to+\infty}\gap_n > \epsilon \right] = \P\left[\bigcup_{N\in\xN}\left\{\inf_{n\geq N} \gap_n>\epsilon\right\} \right]
		\leq \sum_{N\in\xN}\P\left[\inf_{n\geq N} \gap_n>\epsilon \right]
		\leq \sum_{N\in\xN}\P\left[\bigcap_{n\geq N}\left\{\gap_n>\epsilon\right\} \right]
		\\= \sum_{N\in\xN}\lim_{M\to+\infty} \P[G_N^M] \qtext{where}G_N^M \eqdef \bigcap_{n=N}^M\left\{\gap_n>\epsilon\right\}.\label{eq: subadditive prob}
	\end{multline}
	The probability of these events can be bounded inductively for $M\geq N$,
	\begin{align}
		\P(G_N^{M+1}) &= \E\left[\E(\1_{G_N^M\cap\{\gap_{M+1}>\epsilon\}}|\Filtration^M)\right]
		\\&= \E\left[\E(\1_{G_N^M}\cdot\1_{\{\gap_{M+1}>\epsilon\}}|\Filtration^M)\right]
		\\&= \E\left[\1_{G_N^M}\cdot\E(\1_{\{\gap_{M+1}>\epsilon\}}|\Filtration^M)\right] & (G_N^M\in\Filtration^M)
		\\&= \E\left[\1_{G_N^M}\cdot\P(\gap_{M+1}>\epsilon|\Filtration^M)\right] & \text{(def. of $\P$)}
		\\&\leq \E\left[\1_{G_N^M}\cdot(1-\delta(\epsilon))\right] & \text{(def. of $\delta$)}
		\\&= (1-\delta(\epsilon))\P(G_N^M)\ \ldots
		\\&\leq (1-\delta(\epsilon))^{M+1-N}, \label{eq: G_N^M to infty}
	\end{align}
	so $\lim_{M\to+\infty} \P[G_N^M]=0$ for all $N$. This confirms that $\lim_{n\to+\infty}\op{E}(\cm^n) = \op{E}(\cm^*)$ almost-surely, observe
	\begin{align}
		\P(\lim_{n\to+\infty}\op{E}(\cm^n) = \op{E}(\cm^*)) &\geq \P(\liminf_{n\to+\infty}\gap_n \leq 0) & \text{(Theorem~\Rref{thm: inexact FW})}
		\\&= 1-\P(\liminf_{n\to+\infty}\gap_n> 0)
		\\&= 1-\lim_{\epsilon\to0}\P(\liminf_{n\to+\infty}\gap_n> \epsilon) &\text{(monotone convergence)}
		\\&\geq 1 - \lim_{\epsilon\to0}\sum_{N\in\xN}0 & \eqref{eq: subadditive prob}
	\end{align}
	as required.
\end{proof}
While this Theorem~\Rref{thm: inexact stochastic FW} confirms the technical requirements for convergence, the following corollary simplifies these requirements into a more practical format. Assume that the randomness can be summarised for each $n\in\F N$ by
\begin{equation}
	\ep^n = \bar{\LO}(\cm^{n-1},z^n)
\end{equation}
for some approximate linear oracle $\bar{\LO}$, where $z^n\sim Z$ is a random instance of an ambient probability density. The following corollary shows that, if $z^n$ are independent and have a uniformly positive probability of being close to the support of $\LO(\cm^{n-1})$, then the conditions for $\delta$ in Theorem~\Rref{thm: inexact stochastic FW} are greatly simplified. In particular, in the context of this work $z^n$ will be a random discretisation of $\HG$ and $\ep^n$ is the discrete minimiser of the formula \eqref{eq: exact linear oracle}. Theorem~\Rref{thm: inexact stochastic FW} suggests that $z^n$ should need to provide a ``good'' approximation of $\cm^*$, whereas Corollary~\Ref{cor: independent inexact loose} only requires us to approximate $\LO(\cm^n)$. This is easier as we know $\LO(\cm^n)$ has at most singleton support from Lemma~\Rref{lmma: well defined linear oracle}. \rob{The main difference between the $\delta$ in thm 4.4 and cor 4.5 is replacing $\cm^*$ with $\LO(\cm)$. Maybe this notation should be unified. I find the infimum notation more clear but I'm not sure how you write an $S^n$-essential infimum}

\begin{crllr}\label{cor: independent inexact loose}
	Suppose $\ep^n = \bar{\LO}(\cm^{n-1},z^n)$ for some $z^n\sim Z$ and define $\delta\colon\hc{0}{+\infty}\to\ci01$ by 
	\begin{equation}
		\delta(\epsilon) \eqdef \inf_{\cm\in D} \P_{z\sim Z}\left(\IP{\op{E}'(\cm)}{\bar{\LO}(\cm,z)-\LO(\cm)} \leq \epsilon\right).
	\end{equation}
	If $z^{n+1}$ is independent of the filtration $\Filtration^n$ generated by $\{z^k,\cm^k\}_{k=0}^{n}$ for all $n\in\xN$ (\ie\ $z^{n+1}\perp \Filtration^n$), then $\delta$ satisfies \eqref{eq: delta condition}.
\end{crllr}
\begin{lmm}\label{lmma: independent conditional expectation}
	Suppose $X$ is an $\Filtration$-measurable random variable and $Z\perp X, \Filtration$ (\ie\ $Z$ is independent of $X$ and $\Filtration$) is another random variable. Then, for all integrable Borel measurable functions $g$
	\begin{equation}
		\E(g(X,Z)|\Filtration) = G(X) \qtext{where} G(x) \eqdef \E(g(x,Z)).
	\end{equation}
\end{lmm}
This is a standard result in probability theory, see for example \cite[Exercise 9, Chapter 10.1]{Dudley2002}.
\begin{proof}[Proof of Corollary~\Rref{cor: independent inexact loose}.]
	Recall that $\gap_n = \int_\HG [\op{F}'(\cm^n)+w]\xdif[\bar{\LO}(\cm^n,z^{n+1})-\cm^*]$, which is clearly measurable with respect to the filtration generated by $\{\Filtration^n,z^{n+1}\}$.	As $\Filtration^n\perp z^{n+1}$, by Lemma~\Rref{lmma: independent conditional expectation} we therefore have 
	\begin{multline}
		\P(\gap_n\leq\epsilon|\Filtration^n) = \E\left[\1_{\gap_n\leq\epsilon}\,|\Filtration^n\right] = \E\left[\E_{z^{n+1}\sim Z}(\1_{\gap_n\leq\epsilon})\,|\Filtration^n\right] = \E\left[\P_{z^{n+1}\sim Z}(\gap_n\leq\epsilon)\,|\Filtration^n\right]
		\\\geq \inf_{\cm\in D}\P_{z\sim Z}\left(\IP{\op{E}'(\cm)}{\bar{\LO}(\cm,z)-\cm^*}\leq\epsilon\right).
	\end{multline}
	This final value can also be bound from below because, for any $\cm\in D$ and $z\sim Z$,
	\begin{align}
		\IP{\op{E}'(\cm)}{\bar{\LO}(\cm,z)-\cm^*} &= \IP{\op{E}'(\cm)}{\bar{\LO}(\cm,z)-\LO(\cm)} - \IP{\op{E}'(\cm)}{\cm^*-\LO(\cm)}
		\\&\leq \IP{\op{E}'(\cm)}{\bar{\LO}(\cm,z)-\LO(\cm)}.
	\end{align}
	By the monotonicity of probability measures we conclude that $\P(\gap_n\leq \epsilon|\Filtration^n) \geq \delta(\epsilon)$, therefore $\delta$ satisfies \eqref{eq: delta condition} as required.
\end{proof}

\edit{}{With the statement of Corollary~\Rref{cor: independent inexact loose} we can finally prove, for specific examples, that Algorithm~\Rref{alg: inexact FW} with random discretisations of $\HG$ converges to global minimisers of the function $\op{E}$ from Section~\Rref{sec: generalisation}. Consider the Benamou-Brenier example with $\Omega=\oi01^\d$ and, with the discrete-time formulation discussed in Section~\ref{sec: discrete time formulation}, we have $\HG=\bar\Omega^{T+1}$. Note that the simplification does not effect the $\op{F}$ term but it is important for two reasons: it is much easier to randomly sample $\bar\Omega^{T+1}$ than $\Co(\ci01;\bar\Omega)$, and the continuity properties of $w$ are much improved. In particular, from Remark~\Rref{rmk: BB geodesics} we know that $w(\hg) = \alpha+\frac\beta2\sum_{j=1}^T \frac{|\g_j-\g_{j-1}|^2}{t_j-t_{j-1}}$ is in fact continuous, moreover uniformly continuous on the compact set $\bar\Omega^{T+1}$. Also, due to the structure of $\op{F}$ described in \eqref{eq: bounded linear kernels} and \eqref{eq: def of F}, it can be shown that $\enscond{\op{F}'(\cm)+w}{\cm\in D}$ is uniformly equicontinuous. In other words, for any $\epsilon>0$ there is an $r>0$ such that, for all $\hg_1,\hg_2\in\HG$ and $\cm\in D$,
\begin{equation}
	\metric(\hg_1,\hg_2)\equiv \min(2,\norm{\hg_1-\hg_2}_\infty)\leq r\implies  |\op{F}'(\cm)(\hg_1)+w(\hg_1) - \op{F}'(\cm)(\hg_2)+w(\hg_2)|\leq\epsilon.
\end{equation}
Now fix $\cm\in D$ with $\op{supp}(\LO(\cm)) = \{\hg^*\}$ for some $\hg^*\in\HG$ (the alternative case of $\LO(\cm)=0$ is trivial). Then, 
\begin{equation}
	\P_{z\sim Z}\left(\int_\HG \left(\op{F}'(\cm)+w\right)\xdif[\bar{\LO}(\cm,z)-\LO(\cm)] \leq \epsilon\right) \geq \P_{z\sim Z}\left(\inf_{\hg\in z}\norm{\hg-\hg^*}_\infty\leq r\right).
\end{equation}
If we choose $Z$ to be the uniform distribution on $\bar\Omega^{T+1}$, then this probability is lower-bounded by $r^{\d(T+1)}$. This bound is uniform in both $\cm$, therefore $\delta(\epsilon)\eqdef r^{\d(T+1)}$ satisfies the requirements for Corollary~\Rref{cor: independent inexact loose}.}



==> optimal_support.tex <==
%! TEX root = ../main.tex

\section{Support of optimal measures}\label{app: optimal support}
In this section we discuss the continuous-time interpolation of discrete measures. In particular, suppose 
\begin{gather}
	\cm^* \in \argmin_{\cm\in \MC^+(\HG)}\op{E}(\cm),\qquad \op{E}(\cm)= \sum_{j=0}^T\op{F}_j(A_j\cmt{t_j}) + \int_{\HG} w(\hg)\xdif\cm(\hg)
\end{gather}
for lower semi-continuous $w\colon\HG\to\ci{0}{+\infty}$. Note that we have removed the constraint set $D$ in these computations. If there are two terms which are sensitive to the continuous-time interpolation of $\hg$ (rather than just $\hg(t_j)$), then the interpolation must balance both terms. Removing the constraint of $D$, the statement is as follows.

\begin{lmm}\label{app: geodesic support}
Assume that there is a Borel-measurable	mapping $G\colon\HG\to\HG$ such that for all $\hg \in \HG$,
	\begin{equation}
		G(\hg)\in \argmin_{\tilde\hg\in\HG}\enscond{w(\tilde\hg)}{\tilde\hg(t_j)=\hg(t_j)\text{ for all }j=0,\ldots,T}.
	\end{equation}
Then, 
	\begin{equation}
		\text{for a.e. } \hg\in\op{supp}(\cm^*),\qquad w(\hg) = \min_{\tilde\hg\in\HG}\enscond{w(\tilde\hg)}{\tilde\hg(t_j)=\hg(t_j)}.
	\end{equation}
\end{lmm}
\begin{proof}
	
	Since $G$ is Borel-measurable, we may define the image measure $\cm^{**}\eqdef G_\#\cm^*$ by $\cm^{**}(B)=\cm^*(G^{-1}(B))$ for all Borel subset $B$ of $\HG$. Then, since $w\geq 0$ is lower semi-continuous,
	\begin{align}
		\int_{\HG} w \xdif\cm^{**} = \int_{\HG} w(G(\hg)) \xdif\cm^{*}(\hg) 
	\end{align}
	(indeed, the result holds for all continuous bounded function, see \cite[Sec. 5.2]{Ambrosio2008}. One may extend it to $w$ by approximation with an increasing sequence of such functions and the monotone convergence theorem).
	
	Since $\cm^*$ is optimal,
	\begin{align}
		0\geq \op{E}(\cm^*)-\op{E}(\cm^{**}) =\int_{\HG} \left[w(\hg) - w(G(\hg))\right] \xdif\cm^{*}(\hg) 
	\end{align}
	and since $w(\hg)-w(G(\hg))\geq 0$, we deduce that $w(\hg)=w(G(\hg))$ for $\cm^*$-a.e. $\hg \in \HG$.
\end{proof}
For the example in Section~\Rref{sec:BB example}, because $\Omega$ is convex, the map $G(\hg)$ returns the piece-wise linear interpolation of points $\hg(t_0),\ldots,\hg(t_T)$. This is continuous, therefore measurable. 

%\vincent{It is probably possible to prove the existence of $G$. The first thing would be to prove that $\argmin_{\tilde\hg\in\HG}\enscond{w(\tilde\hg)}{\tilde\hg(t_j)=\hg(t_j)}$ is nonempty, using $w$ lsc and coercive. A related issue is lemma A.3}

